On the Origins of Sampling Bias: Implications on Fairness Measurement and Mitigation

Accurately measuring discrimination is crucial to faithfully assessing fairness of trained machine learning (ML) models. Any bias in measuring discrimination leads to either amplification or underestimation of the existing disparity. Several sources of bias exist and it is assumed that bias resulting from machine learning is born equally by different groups (e.g. females vs males, whites vs blacks, etc.). If, however, bias is born differently by different groups, it may exacerbate discrimination against specific sub-populations. Sampling bias, in particular, is inconsistently used in the literature to describe bias due to the sampling procedure. In this paper, we attempt to disambiguate this term by introducing clearly defined variants of sampling bias, namely, sample size bias (SSB) and underrepresentation bias (URB). Through an extensive set of experiments on benchmark datasets and using mainstream learning algorithms, we expose relevant observations in several model training scenarios. The observations are finally framed as actionable recommendations for practitioners.

==> oldexperimentalsetup.tex <==
Having a formal definition of the two variants of sampling bias, namely, sample size bias {\em SSB} and underrepresentation bias {\em URB}, the aim is to analyze bias magnitude in the presence of datasets with various degrees of imbalance. 
%The objective of the experimental analysis is to observe the magnitude of both types of biases, namely, sample size bias {\em SSB} and underrepresenation bias {\em URB} as we change the parameters of data sampling. 
For {\em SSB}, ML models are trained using data samples of increasing sizes and with various imbalance properties. %we train the predictor model using training sets of increasing sizes. 
For {\em URB}, we play rather on the proportions of sensitive groups in the training sample data. \textbf{By comparing model performance on population-sized test sets, the study highlights how underrepresentation bias (URB) and sample size bias (SSB) distort fairness evaluations when based on limited-sized samples.} Next, we study the effect of bias mitigation approaches (preprocessing and in-processing) on the magnitude of both types of bias. Finally, we observe the effect of various types of data augmentation on discrimination. To make comparison with other works in the literature possible, we use three common benchmark datasets, Adult~\cite{kohavi1996scaling}, Compas~\cite{angwin2016machine}, and Dutch Census~\cite{nordholt2004dutch}. %\footnote{We use the same dataset versions and learning algorithms parameters as IBM AIF360~\cite{ibm360}}. 

\subsection{Sample Size Bias (SSB)}

\subsubsection{ Magnitude of Sample Size Bias ({\em SSB})}
\label{sec:exp_ssb}
To observe how sample size bias behaves as the training set size changes, we use the following process. We train ML models using training data samples of increasing size, ranging from $10$ until a given portion of the full dataset size. For example, for COMPAS, we consider sample sizes ranging from $10$ to $2000$. For each sample size value $m$, we repeat the sampling several times ($30$ by default) so that we obtain $30$ samples of each size $m$. Then, we train a different model using each one of the samples so that we obtain $30$ models for each size $m$. We finally compute the discrimination using each model and the returned value is the average discrimination across all models. This procedure gives a sequence of discrimination values indexed by the size. We consider six metrics, %\rut{EO and SD are not accuracy metrics, but fairness metrics. It feels entangled here. Or are we considering $FPR$ difference for both groups? Also are the two groups have equal sample size here? Then the sampling should be done separately for each group. For example for $m=30$, we would sample$ m_1=15$ and $m_0 =15$ } 
namely, $FPR$ (false positive rate), $FNR$ (false negative rate), $EO$ (equal opportunity), {\em AUC} Area Under the Curve, {\em ZOL} (zero one loss), and $SD$ (statistical disparity). We use five classifiers, namely, logistic regression, decision tree, random forest, nearest neighbor, and support vector machine (SVM). For conciseness, only results using logistic regression are reported in the next sections. Results using the remaining learning algorithms can be found in the appendix. % and in the paper online repository.
% \begin{figure}[H]
%     \centering
%     \includegraphics[height=1.9in, width=6in]{Plots/SSB/SSB_Expriment1_non_auc_new_plots_LG.pdf}
%     \includegraphics[height=1.9in, width=6in]{Plots/SSB/SSB_Expriment1_auc_new_plots_LG.pdf}
%      \caption{Magnitude of sample size bias (SSB) when training data is sampled from very discriminative population (postive outcome is 0.9 for privileged group and 0.1 for unprivileged group).}
%     \label{fig:ssb_lg_veryDisc}
% \end{figure}
\subsubsection{{\em SSB} when training data is imbalanced} To analyze further the behavior of {\em SSB}, we focus on the case of extreme imbalance between the protected groups. For instance, for Adult dataset, we consider a version where the rate of positive outcome is $0.9$ for the privileged group (males) and $0.1$ for the unprivileged group (females).
\subsection{Uderrepresentation Bias (URB)}

\subsubsection{Magnitude of discrimination in {\em URB} experiment}
A bias in measuring discrimination may exacerbate the discrimination but also may attenuate it. A similar experiments to Section~\ref{sec:exp_ssb} shows that the effect of {\em URB} depends on how much discrimination there is in the data initially. Figure~\ref{fig:URB_veryBiased} depicts the result of a set of experiments carried out on a significantly imbalanced version of the Adult dataset. In such versions, the rate of positive outcome is 90\% for the privileged group and 10\% for the unprivileged group. That is, discrimination is initially very significant. To see the effect of underrepresentation on discrimination, we train models using the same splitting values as above and considering extreme splitting values (e.g. $0.001$ vs $0.99$, $0.002$ vs $0.98$, etc.).

 \subsubsection{Magnitude of underrepresentation bias ({\em URB})} The aim for underrepresentation bias experiment is to observe the magnitude of {\em URB} while the ratio of the sensitive groups in the training set is changing. We consider different values of the splitting $\frac{m_1}{m_0}$ (see Definition~\ref{def:urb}) (e.g. $0.1$ vs $0.9$, $0.2$ vs $0.8$, etc.). However, as {\em URB} is more significant for extreme disparities in group size, we focus more on extreme splitting values (e.g. $0.001$ vs $0.99$, $0.002$ vs $0.98$, etc.). A similar behavior has been observed previously by Farrand et al.~\cite{farrand2020neither}. Assuming a fixed sample size (e.g. $1000$), for each splitting value, we sample the data so that the proportions of sensitive groups (e.g. male vs female) match the splitting value. Similarly to the {\em SSB} experiment, we repeat the sampling several times ($30$ by default) for the same splitting value. Then, we train a different model using each one of the samples so that we obtain $30$ models for each splitting value $\frac{m_1}{m_0}$. The discriminations obtained using the different models are then averaged across all models. We finally obtain a sequence of discrimination values indexed by the splitting value.
\subsection{Bias Mitigation}

\subsubsection{Pre-processing and In-processing} First, Reweighing~\cite{kamiran2012data} tries to mitigate the effects of discrimination on the learned model by adjusting the weights of training samples based on group representation. This method ensures that groups that are underrepresented in the training data are given a higher weight during the learning process, thus improving the model's ability to learn from these groups effectively. We applied reweighing during the preprocessing stage to all datasets before model training. Second, GerryFairClassifier~\cite{kearns2019empirical} which introduces fairness constraints directly into the learning process. This in-processing method works by adjusting the optimization objective of the model to account for fairness criteria, effectively reducing disparities across sensitive groups while still striving for predictive accuracy. 
To observe very clearly the effect of Reweighing pre-processing mitigation approach on the training dataset size, we consider the same significantly unfair version of the benchmark datasets as in Figure~\ref{fig:SSB_disc_LG_biased}. That is, a version where the rate of positive outcome is 0.9 for the privileged group (e.g. male) and 0.1 for the unprivileged group (e.g. female).

\subsubsection{Random Data Augmentation}
In the following, we devise simple experiments to observe the effect of populating the data with more samples collected from the same population as the existing data. Using the same benchmark datasets, the aim is to train models based on an increasing number of under represented group samples while keeping the privileged group portion unchanged. For the particular case of Dutch Census dataset, we train models using a set composed of a fixed $100$ privileged group (male) samples and an increasing number of protected group (female) samples starting from $2$ until $100$ (perfect balance between groups). Similarly to the {\em SSB} and {\em URB} experiments, it turns out that the magnitude of discrimination is manifested more with extreme values of protected groups sizes (typically less than $100$) which explains the specific sample sizes considered. 


==> preliminaries.tex <==
\section{Method} \label{app:METHOD}

% \subsection{Datasets and Metrics}\label{app:metrics}
% To explore the effects of SSB and URB on ML fairness, we utilized three benchmark datasets:\\ Adult \cite{kohavi1996scaling}, COMPAS \cite{angwin2016machine}, and Dutch Census \cite{laan2015dutch} . These datasets were chosen because they contain rich demographic information that enables detailed fairness analysis across sensitive groups such as gender and race.
% \begin{table}[ht]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \textbf{Dataset}           & \textbf{Adult }  & \textbf{COMPAS }  & \textbf{Dutch Census }  \\ \hline
% \textbf{Date of Publication} & 1996       & 2016       & 2001             \\ \hline
% \textbf{Number of Instances} & 48,842                  & 6,172                    & 60,420                        \\ \hline
% \textbf{Number of Attributes} & 14  & 14  & 10 \\ \hline
% \textbf{Sensitive Attribute} & Gender                     & Race                     & Gender                           \\ \hline
% \textbf{Label}              & Income (\(>50K, <50K\))   & Recidivism (Risk of Reoffending) & Occupation                   \\ \hline
% \end{tabular}
% \vspace{2mm}
% \caption{Summary of Datasets}
% \end{table}



% The following metrics are used to evaluate fairness in our experiments:
% \begin{itemize}
%     \item \textbf{False Positive Rate (FPR) :} It is the proportion of negative instances that are incorrectly classified as positive. High disparities in FPR across groups indicate bias.
%     \begin{equation}\label{equation:fpr}
%     \text{FPR} = \frac{FP}{FP + TN}
% \end{equation}
%     \item \textbf{Equal Opportunity (EO):} It is the difference in true positive rates between sensitive groups, assessing the fairness of positive predictions.
%     \begin{equation}\label{equation:eo}
%     \text{EO} = \frac{TP}{TP + FN}
% \end{equation}
%     \item \textbf{Zero-One Loss (ZOL):} It is the overall misclassification rate, which can be impacted by bias if certain groups have systematically higher misclassification rates.
%     \begin{equation}
%     \label{equation:zol}
% \text{Zero-One Loss}(y, \hat{y}) = 
% \begin{cases} 
% 1 & \text{if } y \neq \hat{y} \\ 
% 0 & \text{if } y = \hat{y} 
% \end{cases}
% \end{equation}
%     \item \textbf{Statistical Disparity (SD):}It measures the difference in selection rates between groups, and is useful for assessing disparate impact.
%     \begin{equation}\label{equation:sd}
%     \text{SD} = P(\hat{Y}=1 \mid \text{Unprivileged}) - P(\hat{Y}=1 \mid \text{Privileged})
% \end{equation}
%     \item \textbf{Area Under the Curve (AUC):}It evaluates the trade-off between sensitivity and specificity, and is useful for understanding how bias affects the overall model performance.
%     \begin{center}
 
% \end{center}
% \end{itemize}

\subsection{Experimental Set-up}\label{app:methods}

This study investigates the impact of sample size bias ({\em SSB}) and underrepresentation bias ({\em URB}) on fairness evaluations, particularly in datasets with varying levels of imbalance. {\em SSB} is analyzed by training ML models with datasets of increasing sizes, while {\em URB} is studied by varying the representation of sensitive groups in training data. Model performance is evaluated on population-sized test sets to demonstrate how these biases distort fairness assessments when fairness metrics are applied to smaller test sets or test sets with imbalances different from that of the population. The study also examines the effect of bias mitigation techniques (pre-processing and in-processing) and data augmentation on discrimination. 

% Experiments use three benchmark datasets: Adult~\cite{kohavi1996scaling}, COMPAS~\cite{angwin2016machine}, and Dutch Census~\cite{nordholt2004dutch}. We use following metrics to measure discrimination: difference in  $FPR$ (false positive rate), equal opportunity~\cite{hardt2016equality}, difference in $ZOL$ (zero-one loss), difference in $AUC$ (area under the curve), and statistical disparity~\cite{dwork2012fairness}. Five classifiers are evaluated: logistic regression, decision tree, random forest, nearest neighbor, and SVM. Results for logistic regression are presented; others are included in the appendix.%, and, for regression problems, difference in $MSE$ (mean squared error). For the latter, we use previous results in the literature~\cite{chen2018,domingos2000} to decompose the discrimination into noise, bias, and variance. 


\subsubsection{Sample Size Bias (SSB)}

%\subsubsection{ Magnitude of Sample Size Bias ({\em SSB})}
\label{sec:exp_ssb}
To measure SSB, ML models are trained on datasets with increasing sample sizes (e.g., from 10 to 2000 samples for COMPAS). For each size $m$, 30 samples are drawn, and a separate model is trained on each. 
% The average discrimination across these models is computed for metrics including $FPR$ (false positive rate), $FNR$ (false negative rate), $EO$ (equal opportunity), {\em AUC} (area under the curve), {\em ZOL} (zero-one loss), and $SD$ (statistical disparity). 
%\subsubsection{{\em SSB} when training data is imbalanced} 
To analyze further the behavior of {\em SSB}, we focus on the case of extreme imbalance between the protected groups. For example, for the adult dataset, we consider a version in which the positive outcome rate is $0.9$ for the privileged group (males) and $0.1$ for the unprivileged group (females).

\subsubsection{Uderrepresentation Bias (URB)}
%The behavior of SSB is further analyzed under extreme imbalances. For example, in the Adult dataset, we consider scenarios where the positive outcome rate is 0.9 for the privileged group (males) and 0.1 for the unprivileged group (females). 

%\subsubsection{Magnitude of underrepresentation bias ({\em URB})} 

The aim for underrepresentation bias experiment is to observe the magnitude of {\em URB} while the ratio of the sensitive groups in the training set is changing. We consider different values of the splitting $\frac{m_1}{m_0}$ (see Definition~\ref{def:urb}) (e.g. $0.1$ vs $0.9$, $0.2$ vs $0.8$, etc.). However, as {\em URB} is more significant for extreme disparities in group size, we focus more on extreme splitting values (e.g. $0.001$ vs $0.99$, $0.002$ vs $0.98$, etc.). A similar behavior has been observed previously by Farrand et al.~\cite{farrand2020neither}. Assuming a fixed sample size (e.g. $1000$), for each splitting value, we sample the data so that the proportions of sensitive groups (e.g. male vs female) match the splitting value. Similarly to the {\em SSB} experiment, we repeat the sampling several times ($30$ by default) for the same splitting value. Then, we train a different model using each one of the samples so that we obtain $30$ models for each splitting value $\frac{m_1}{m_0}$. The discriminations obtained using the different models are then averaged across all models.
Similarly to {\em SSB} experiment, to analyze further the behavior of {\em URB} in presence of significant discrimination, we focus on the case of extreme imbalance between the protected groups. For example, for the adult dataset, we consider a version in which the positive outcome rate is $0.9$ for the privileged group (males) and $0.1$ for the unprivileged group (females).


% URB is analyzed by varying the ratio of sensitive groups in training data. For extreme imbalances, splitting ratios such as $0.001$ vs $0.99$ and $0.002$ vs $0.98$ are used. Assuming a fixed sample size (e.g., 1000), data is sampled to match each ratio, and models are trained on 30 samples per ratio. The average discrimination is computed across these models.

% \subsubsection{The Effect of discrimination on {\em URB}}
% The effect of URB depends on the initial level of discrimination in the data. For instance, in a highly imbalanced version of the Adult dataset ($90\%$ positive outcomes for the privileged group vs. $10\%$ for the unprivileged group), experiments demonstrate how URB exacerbates or attenuates discrimination.
 

\subsubsection{Bias Mitigation}
Next, we focus on the effect of both types of bias ({\em SSB} and {\em URB}) on discrimination when bias mitigation approaches are used in model training. Several bias mitigation approaches have been developed in the few last years~\cite{dunkelau2019fairness,hort2024bias,siddique2023survey}. Most of these approaches fall into two categories. First pre-processing techniques which try to transform the data so that the underlying discrimination is removed. Second, in-processing techniques which try to modify the learning algorithms in order to remove discrimination during the model training process. We consider one representative technique from each approach. First, Reweighing~\cite{kamiran2012data} tries to mitigate the effects of discrimination on the learned model by adjusting the weights of training samples based on group representation. This method ensures that groups that are underrepresented in the training data are given a higher weight during the learning process, thus improving the model's ability to learn from these groups effectively. We applied reweighing during the preprocessing stage to all datasets before model training. Second, GerryFairClassifier~\cite{kearns2019empirical} which introduces fairness constraints directly into the learning process. This in-processing method works by adjusting the optimization objective of the model to account for fairness criteria, effectively reducing disparities across sensitive groups while still striving for predictive accuracy. 


% \subsubsection{Pre-processing and In-processing} 
% Two mitigation techniques are examined:
% \begin{itemize}
%     \item  Reweighing~\cite{kamiran2012data}: Adjusts training sample weights to counteract underrepresentation.
%     \item GerryFairClassifier~\cite{kearns2019empirical}: Incorporates fairness constraints into model optimization.
% \end{itemize}
% Experiments use significantly biased dataset versions (e.g., 0.9 positive outcome rate for privileged groups and 0.1 for unprivileged groups) to evaluate these techniques.

\subsubsection{Data Augmentation}

The natural approach to address sampling bias is to use more data for training, in particular for the under-represented groups. Obtaining more data is possible either through data augmentation or data collection. Data augmentation is the process of using the available data to generate more samples. In turn, this can be done in two ways: oversampling or creating synthetic samples. Oversampling consists in duplicating existing samples to balance the data. A simple variant is to randomly duplicate samples from the under represented group. Creating synthetic samples, on the other hand, is typically done using SMOTE~\cite{chawla2002smote}. %SMOTE creates synthetic samples based on the k-nearest neighbors of every sample of the under represented group. 
Both techniques of data augmentation try to balance data by adding artificially generated samples. While this artificial manipulation may reduce discrimination between sensitive groups, it can lead to models which are not faithful to reality. When it is possible, collecting more data is more natural and reflects better reality. The approach is simple: if a sensitive group is under represented, collect more samples of that group. Unlike data augmentation, whose effect on discrimination has been the topic of a number of papers, in particular related to computer vision (e.g.~\cite{pastaltzidis2022data,yucer2020exploring, zhang2020towards,xu2020investigating,Wang2018BalancedDA,wang2020towards}), the impact of  of collecting more samples on discrimination has not been well studied in the literature. 

We devise simple experiments to observe the effect of populating the data with more samples collected from the same population as the existing data. Using the same benchmark datasets, the aim is to train models based on an increasing number of one protected group while keeping the other group portion unchanged. %For the particular case of Dutch Census dataset, we train models using a set composed of a fixed $100$ privileged group (male) samples and an increasing number of protected group (female) samples starting from $2$ until $100$ (perfect balance between groups).
For instance, for the Dutch Census dataset, models are trained with $100$ privileged group samples and increasing protected group samples (from $2$ to $100$). We use 3-fold cross-validation and randomly generate $50$ different samples for every size value. In the selective data augmentation variant of the same experiment, additional samples are collected exclusively from the protected group with positive outcomes. This behavior is compared to two other augmentation strategies: randomly collecting more protected group samples and randomly collecting more unprotected group samples. In all three cases, the importance of the sensitive feature (e.g., sex) in prediction, as measured by SHAP explanations~\cite{lundberg2017unified}.

% \subsubsection{Random Data Augmentation}
% We assess the impact of adding more samples from underrepresented groups while keeping privileged group sizes fixed. For the Dutch Census dataset, models are trained with 100 privileged group samples and increasing protected group samples (from 2 to 100). We use 3-fold cross-validation and randomly generate $50$ different samples for every size value. Discrimination is most pronounced for extreme underrepresentation, justifying the focus on small sample sizes.

% \subsubsection{Selective Data Augmentation}

% In this experiment the additional samples are collected exclusively from the protected group with positive outcomes. This behavior is compared to two other augmentation strategies: randomly collecting more protected group samples and randomly collecting more unprotected group samples.
% In all three cases, the importance of the sensitive feature (e.g., sex) in prediction, as measured by SHAP explanations~\cite{lundberg2017unified}.



==> text-03-relatedwork.tex <==

An exhaustive list of sources of bias can be found in the survey paper of Mehrabi et al.~\cite{mehrabi2021survey} where the authors categorized them into three categories: biases in the data (measurement, representation\footnote{The term representation bias in the context of computer vision denotes a different type of bias: the presence of potential ``shortcuts'' that a model can exploit to accurately predict the label without learning the underlying task~\cite{li2019repair}. A simple example is when the background environment of a picture can be used to recognize the object of interest.}, etc.), biases in the algorithm (algorithmic, evaluation, etc.), and biases introduced by users (historical, self-selection, etc.). This paper focuses on biases in the first category. Suresh et al.~\cite{suresh2019framework}, however, categorized the sources of bias into five categories depending on where in the machine learning pipeline a bias may be introduced. Although they provide a framework for the machine learning pipeline transformations, sources of bias that can impact the transformations are only described informally (Figure 2 in~\cite{suresh2019framework}). Similarly, Hellstrom et al.~\cite{hellstrom2020bias} propose a taxonomy of the sources of bias while categorizing them on the basis of the machine learning pipeline. The main limitation of all previous work on sources of bias is the absence of formal definitions of biases. Therefore, these papers did not include an analysis of the correlation between the magnitude of the bias and the extent of the discrimination.

Sampling bias is related to the known problems of (1) learning using a limited size training set and (2) learning using imbalanced data~\cite{he2009learning}. Chen et al.~\cite{chen2018} studied the effect of the training set sample size on discrimination. They used two discrimination metrics, namely, false positive rate (FPR) and false negative rate (FNR). They found that discrimination according to FNR is much more sensitive to sample size than FPR. To address the problem of imbalanced data, Yan et al.~\cite{yan2020fair} compared existing techniques for balancing data and found that while they achieve better prediction, they tend to exacerbate discrimination. Farrand et al.~\cite{farrand2020neither} focused on the impact of using imbalanced data on the accuracy and fairness of the obtained model while learning with privacy (differencial privacy (DP)) constraints. They found that data imbalance has little effect on discrimination (equal opportunity and statistical disparity) until the imbalance between sensitive groups becomes extreme (e.g. $99.9\%$ vs $0.1\%$). Interestingly, the impact is more important for DP-learned models than with non-DP models.

Machine learning loss/error has been first decomposed into bias and variance by Dietterich and Kong~\cite{dietterich1995}. The decomposition did not distinguish between variance and noise and considered noise as part of variance (variance is defined as the difference between loss and bias). They illustrated the decomposition for regression and for classification problems but only for individual examples. Domingos~\cite{domingos2000} distinguished between noise and variance and extended the decomposition to the expectation over all samples. He considered three loss functions, namely, squared loss, absolute loss, and zero-one loss. For the experimental analysis, Domingos focused on decision trees and k-nearest neighbor (KNN) learning algorithms and studied the effect of some parameters on the loss, namely, pruning parameters, level of the tree, number of rounds in boosting, and the k parameter in KNN. Chen et al.~\cite{chen2018} leveraged these previous results to decompose the discrimination between sensitive groups. They considered two types of loss functions, namely, zero-one loss for classification and squared loss for regression. They also studied the effect of increasing training data size on the discrimination. To this end, they assumed that the losses (population and group-specific) have an inverse power-low behavior asymtotically. This allows to predict the discrimination level if training data is augmented with additional samples.

Additional data collection for minority group or data augmentation is well known as a fairness remedy for imbalanced data, particularly in computer vision~\cite{pastaltzidis2022data,yucer2020exploring,zhang2020towards,xu2020investigating,Wang2018BalancedDA,wang2020towards, buolamwini2018gender}. Data augmentation can be split into two approaches. First is replicating or generating additional synthetic data points for the minority group that follows the same distribution~\cite{iosifidis2018dealing}. Second approach for data augmentation consists of selectively~\textit{balancing} the data with respect to the positive label and the sensitive group\cite{burns2018women}. In this study we explore the increase in data size, or the size of a sensitive minority group by adding additional samples from the same population distribution, which is closer to the first approach or additional data collection.


==> text-05-decomposition.tex <==

\label{sec:decomposition}

Domingos~\cite{domingos2000} showed that if a learning algorithm $\mathcal A$ learns a function $\mathcal{A}(\mathcal{S}) = \hat{f}_{\mathcal{S}}$ based on a training set $\mathcal{S} \in \mathfrak{S}$, then the expected loss between the prediction $\hfs(\bx)$ and the true value $f(\bx)$ can be decomposed into noise, bias, and variance. In particular, for squared loss,
\begin{equation}L^{SL}(\hfs(\bx),f(\bx)) = N^{SL}(\bx) + B^{SL}(\bx) + V^{SL}(\bx)\label{eq:decomposition0}\end{equation}
where 
\begin{itemize}
    \item[$\circ$] $N^{SL}(\bx) = L^{SL}(f^{*}(\bx),f(\bx))$
    \item[$\circ$] $B^{SL}(\bx) = L^{SL}(\bhf(\bx),f^{*}(\bx))$
    \item[$\circ$] $V^{SL}(\bx) = \ep_{\mathcal{S} \in \mathfrak{S}}[L^{SL}(\hfs(\bx),\bhf(\bx))]$
\end{itemize}
The loss decomposition can be illustrated as follows:

\begin{tikzpicture}
\matrix[row sep=-0.2cm,column sep=0.2cm] {%
    % First row:
    \node (p1) {$f(\bx)$};   &&&& \node (p2) {$f^{*}(\bx)$}; &&&& \node (p3) {$\bhf(\bx)$}; &&&& \node (p4) {$\hfs(\bx)$}; \\
    && \node (p5) {$Noise$};   &&&& \node (p6) {$Bias$}; &&&& \node (p7) {$Variance$}; &&; \\
};
\draw   (p1) edge [<->,>=stealth,shorten <=2pt, shorten >=2pt, thick] (p2);
\draw   (p2) edge [<->,>=stealth,shorten <=2pt, shorten >=2pt, thick] (p3);
\draw   (p3) edge [<->,>=stealth,shorten <=2pt, shorten >=2pt, thick] (p4);       
\end{tikzpicture}

For Zero-One loss ($L^{ZO}$), Equation~\ref{eq:decomposition0} holds also but with coefficients different than $1$ for the noise and variance terms. However, it does not hold for the absolute loss ($L^{AL}$)\footnote{Alternatively, upper and lower bounds are possible.}~\cite{domingos2000}


% \begin{figure}[h]  
% \centering 








\subsection{Decomposing Discrimination}



Chen et al.~\cite{chen2018} showed that the accuracy/cost metric $C^{\bullet}_a(\Yhs)$ as well as the discrimination $Disc^{\bullet}(\Yhs)$ can be decomposed into noise, bias, and variance components. In particular, for MSE, 

\begin{equation}
    C^{\tin{MSE}}_a(\Yhs) = \overline{N}_{a}^{\tin{SL}}(\Yhs) + \overline{B}_{a}^{\tin{SL}}(\Yhs) + \overline{V}_{a}^{\tin{SL}}(\Yhs) \label{eq:LDecomp0}
\end{equation}
where:
\begin{itemize}
    \item[$\circ$] $\overline{N}_{a}^{\tin{SL}}(\Yhs) = \ep_{\bx \in \mathcal{X}} [N^{SL}(\bx)|A=a]$ 
    \item[$\circ$] $\overline{B}_{a}^{\tin{SL}}(\Yhs) = \ep_{\bx \in \mathcal{X}} [B^{SL}(\bx)|A=a]$ 
    \item[$\circ$] $\overline{V}_{a}^{\tin{SL}}(\Yhs) = \ep_{\bx \in \mathcal{X}} [(1-2\times B^{SL}(\bx))\times V^{SL}(\bx)|A=a]$    
\end{itemize}
The last term ($V_a(\Yhs)$) is called \textit{net variance}~\cite{domingos2000}. Consequently,
\begin{equation}
    Disc^{\tin{MSE}}(\Yhs) = (\overline{N}_{a_1}^{\tin{SL}}(\Yhs) - \overline{N}_{a_0}^{\tin{SL}}(\Yhs)) + (\overline{B}_{a_1}^{\tin{SL}}(\Yhs) - \overline{B}_{a_0}^{\tin{SL}}(\Yhs)) + (\overline{V}_{a_1}^{\tin{SL}}(\Yhs) - \overline{V}_{a_0}^{\tin{SL}}(\Yhs)) \label{eq:discDecomp0}
\end{equation}

 %Other notions of fairness can be defined using different accuracy cost functions such as $FPR$, $FNR$, and Zero-One loss ($ZOL$). 
 The decomposition of Equation~\ref{eq:discDecomp0} will also hold for $Disc^{\tin{FPR}}(\Yhs)$, $Disc^{\tin{EO}}(\Yhs)$, and $Disc^{\tin{ZOL}}(\Yhs)$ but with coefficients different than $1$ for the noise and variance terms~\cite{chen2018}.

\subsection{Decomposing $SSB$ and $URB$}
The variant $SSB_M^{\bullet}(\mathcal{A},\mathcal{S}_m)$ (Eq.~\ref{eq:ssb2}) of sample size bias has the advantage that it can be decomposed into bias and variance. The decomposition for the $MSE$ metric is as follows.
\begin{theorem}
\label{th:ssb_decomp}
$SSB_M^{\tin{MSE}}(\mathcal{A},\mathcal{S}_m)$ can be decomposed into bias and variance components as follows:
\begin{align}
SSB_M^{\tin{MSE}}(\mathcal{A},\mathcal{S}_m) & = \overline{B}^{SL}_{a_1}(\hYsm) - \overline{B}^{SL}_{a_1}(\bhY_M) - (\overline{B}^{SL}_{a_0}(\hYsm) - \overline{B}^{SL}_{a_0}(\bhY_M)) \nonumber \\
& + \overline{V}^{SL}_{a_1}(\hYsm) - \overline{V}^{SL}_{a_1}(\bhY_M) - (\overline{V}^{SL}_{a_0}(\hYsm) - \overline{V}^{SL}_{a_0}(\bhY_M)) \nonumber   
\end{align}
\end{theorem}
\begin{proof}
The proof follows from Equation~\ref{eq:LDecomp0} and from assuming that the optimal predictor $Y^{*}$ coincides with the true value $Y$ and hence noise is $0$ \footnote{We follow previous work (Domingos~\cite{domingos2000} and Kohavi and Wolpert~\cite{kohavi1996bias}) in assuming a zero noise.}. 
\end{proof}

$URB^{\bullet}(\mathcal{A},\mathcal{S}_{\frac{m_1}{m_0}})$ (Equation~\ref{eq:urb2}) can also be decomposed into bias and variance components. The decomposition for the $MSE$ metric is as follows.
\begin{theorem}
\label{th:urb_decomp}
\begin{align}
    URB^{\tin{MSE}}(\mathcal{A},\mathcal{S}_{\frac{m_1}{m_0}}) & = \overline{B}^{SL}_{a_1}(\hYmm) - \overline{B}^{SL}_{a_1}(\bhYmmp) - (\overline{B}^{SL}_{a_0}(\hYmm) - \overline{B}^{SL}_{a_0}(\bhYmmp)) \nonumber \\
& + \overline{V}^{SL}_{a_1}(\hYmm) - \overline{V}^{SL}_{a_1}(\bhYmmp) - (\overline{V}^{SL}_{a_0}(\hYmm) - \overline{V}^{SL}_{a_0}(\bhYmmp)) \nonumber 
\end{align}
\end{theorem}
\begin{proof}
The same as Theorem~\ref{th:ssb_decomp}.
\end{proof}

%$ = Disc^{\bullet}(\hYmm) - Disc^{\bullet}(\bhYmmp)$ \label{eq:urb2}




==> text-065-RelatedApplication.tex <==



